Formally Verified Certification of Unsolvability of Temporal Planning Problems

We present an approach to unsolvability certification of temporal planning. Our approach is based on encoding the planning problem into a network of timed automata, and then using an efficient model checker on the network followed by a certificate checker to certify the output of the model checker. Our approach prioritises trustworthiness of the certification: we formally verify our implementation of the encoding to timed automata using the theorem prover Isabelle/HOL and we use an existing certificate checker (also formally verified in Isabelle/HOL) to certify the model checking result.

==> enumitem-unboxed-join.tex <==
\RequirePackage{etoolbox}
\makeatletter
\newcount\enit@ubx@listcnt   %
\newcount\enit@ubx@itemcnt   %
\def\enit@ubx@last{0}
\def\enit@noboxitem[#1]{%
  \if@newlist
    \leavevmode %
    \global\@newlistfalse
    \global\advance\enit@ubx@listcnt\@ne
    \edef\enit@ubx@id{\the\enit@ubx@listcnt}%
    \enit@ubx@itemcnt\z@
    \expandafter\ifx\csname enit@ubx@last@\enit@ubx@id\endcsname\relax
      \def\enit@ubx@last{0}%
    \else
      \edef\enit@ubx@last{\csname enit@ubx@last@\enit@ubx@id\endcsname}%
    \fi
  \else
    \ifhmode
      \unskip
      \ifx\enit@itemjoin@s\relax
        \enit@itemjoin
      \else
        \ifnum\numexpr\enit@ubx@itemcnt+1\relax=\enit@ubx@last\relax
          \enit@itemjoin@s
        \else
          \enit@itemjoin
        \fi
      \fi
    \else
      \noindent
    \fi
  \fi
  \advance\enit@ubx@itemcnt\@ne
  \if@noitemarg
    \@noitemargfalse
    \if@nmbrlist
      \refstepcounter{\@listctr}%
    \fi
  \fi
  \mbox{\makelabel{#1}}%
  \enit@afterlabel
  \ignorespaces}
\let\enit@ubx@orig@endinlist\enit@endinlist
\def\enit@endinlist{%
  \ifenit@boxmode\else
    \ifx\enit@ubx@id\@undefined\else
      \immediate\write\@auxout{\string\global\string\@namedef{enit@ubx@last@\enit@ubx@id}{\the\enit@ubx@itemcnt}}%
    \fi
  \fi
  \enit@ubx@orig@endinlist}
\patchcmd{\enit@inlist}%
  {\PackageWarning{enumitem}{itemjoin* discarded in mode unboxed\MessageBreak}}%
  {}{}{\PackageWarning{enumitem-unboxed}{could not silence the itemjoin* warning}}
\makeatother

